In-Home Daily-Life Captioning Using Radio Signals

This paper aims to caption daily life --i.e., to create a textual description of people's activities and interactions with objects in their homes. Addressing this problem requires novel methods beyond traditional video captioning, as most people would have privacy concerns about deploying cameras throughout their homes. We introduce RF-Diary, a new model for captioning daily life by analyzing the privacy-preserving radio signal in the home with the home's floormap. RF-Diary can further observe and caption people's life through walls and occlusions and in dark settings. In designing RF-Diary, we exploit the ability of radio signals to capture people's 3D dynamics, and use the floormap to help the model learn people's interactions with objects. We also use a multi-modal feature alignment training scheme that leverages existing video-based captioning datasets to improve the performance of our radio-based captioning model. Extensive experimental results demonstrate that RF-Diary generates accurate captions under visible conditions. It also sustains its good performance in dark or occluded settings, where video-based captioning approaches fail to generate meaningful captions. For more information, please visit our project webpage: http://rf-diary.csail.mit.edu

==> arxiv eccv/source/abstract.tex <==
%Event captioning aims to describe events and people's activities during a period of time. In particular, events captioning in people's home can empower various applications such as security, smart home and health care. However, previous event captioning methods mostly focus on generating descriptions based on RGB videos, which is vulnerable to poor-light conditions, background noise and can be privacy invasive. In this paper, we introduce \name, a system that describes in-home events based on radio signals.
%\name~takes radio frequency (RF) signals and floor-maps as inputs. It first generate 3D human skeletons from RF signals. Then it combines the extracted skeletons and the floor-map to generate intermediate features that lie in the same space of features from RGB videos, and use those features to generate sentences that accurately describe various events. By aligning the features from skeletons+floor-maps and RGB videos in the latent space, we transfer the knowledge from RGB video captioning to the RF-caption model and allow it to learn from a rather small dataset. 
%Extensive experimental results demonstrate that RF-Caption can generate accurate sentence descriptions under visible conditions, and obtain similar results under dark conditions where video-based captioning approaches fails to generate meaningful captions.


%Daily life captioning aims to describe people's in-home activities in sentences. It can empower various applications such as smart home and healthcare. However, people will not be willing to deploy cameras in their homes as required by conventional video captioning, and using cameras to cover the whole home can introduce large overhead. In this paper, we introduce \name, a system that enables daily life captioning in a more effective and acceptable way by using ubiquitous radio frequency (RF) signals. To help model people's interaction with in-home objects, we use floor-maps to provide additional information about the surrounding environment. \name~first generates 3D human skeletons from RF signals. Then it combines the features of skeletons and floor-maps to generate accurate natural language descriptions. We further propose a multi-modal feature alignment training scheme to transfer the knowledge from video-based captioning to RF-caption which allow it to learn from a rather small dataset. Extensive experiment results demonstrate that RF-Caption can generate accurate sentence descriptions under visible conditions, and obtain similar results under dark or occluded conditions where video-based captioning approaches fails to generate meaningful captions.

%This paper aims to caption daily life --i.e., to create a textual description of people's activities and interactions with objects in their homes.  Addressing this problem requires novel methods beyond traditional video captioning, as most people would have privacy concerns about deploying cameras throughout their homes. We introduce \name, a new model for captioning daily life by analyzing the radio signal in the home along with the home's floormap. \name\ is more privacy preserving than RGB-based captioning. Further, since it operates with radio signals, it can observe and caption people's life through walls and occlusions and in dark settings. In designing \name, we exploit the ability of radio signal to capture people's 3D dynamics. We also use a multi-modal feature alignment training scheme in order to leverage existing video-based captioning datasets to improve the performance of our radio-based captioning model. Extensive experimental results demonstrate that \name\ generates accurate sentence descriptions under visible conditions, and sustains its good performance in dark or occluded settings, where video-based captioning approaches fail to generate meaningful captions.

This paper aims to caption daily life --i.e., to create a textual description of people's activities and interactions with objects in their homes.  Addressing this problem requires novel methods beyond traditional video captioning, as most people would have privacy concerns about deploying cameras throughout their homes. We introduce \name, a new model for captioning daily life by analyzing the privacy-preserving radio signal in the home with the home's floormap. \name\ can further observe and caption people's life through walls and occlusions and in dark settings. In designing \name, we exploit the ability of radio signals to capture people's 3D dynamics, and use the floormap to help the model learn people's interactions with objects. We also use a multi-modal feature alignment training scheme that leverages existing video-based captioning datasets to improve the performance of our radio-based captioning model. Extensive experimental results demonstrate that \name\ generates accurate captions under visible conditions. It also sustains its good performance in dark or occluded settings, where video-based captioning approaches fail to generate meaningful captions.\footnote{For more information, please visit our project webpage: \href{http://rf-diary.csail.mit.edu}{\color{magenta}http://rf-diary.csail.mit.edu}}

 



==> arxiv eccv/source/conclusion.tex <==
\section{Conclusion}
In this paper, we introduce \name, a system that enables in-home daily-life captioning using RF signals and floormaps. 
We also introduce the combination of RF signal and floormap as new complementary input modalities, and propose a feature alignment training scheme to transfer the knowledge from large video-captioning dataset to \name. 
Extensive experimental results demonstrate that \name~can generate accurate descriptions of in-home events even when the environment is under poor lighting conditions or has occlusions.  We believe this work paves the way for many new applications in health monitoring and smart homes. 
%Future works can be generating everyday diary for people or sending alerts based on the generated captions.

==> arxiv eccv/source/experiment-3.tex <==
\section{Experiments}
\textbf{(a)~Datasets:~~}
\label{sec:dataset}
We collect a new dataset named RF Captioning Dataset (RCD). It provides synchronized RF signals, RGB videos, floormaps, and human-labeled captions to describe each event. We generate floormaps using a commercial laser meter. The floormaps are marked with  the following objects: cabinet, table, bed, wardrobe, shelf, drawer, stove, fridge, sink, sofa, television, door, window, air conditioner, bathtub, dishwasher, oven, bedside table. We use a radio device to collect RF signals, and a multi-camera system to collect multi-view videos, as the volunteers perform the activities. The synchronized radio signals and videos have a maximum synchronization error of 10 ms. The multi-camera system has 12 viewpoints to allow for accurate captioning even in cases where some viewpoints are occluded or the volunteers walk from one room to another room. 

To generate captions, we follow the method used to create the Charades dataset~\cite{sigurdsson2016hollywood} --i.e., we first  generate instructions similar to those used in Charades, ask the volunteers to perform activities according to the instructions, and record the synchronized RF signals and multi-view RGB videos. We then provide each set of multi-view RGB videos to Amazon Mechanical Turk (AMT) workers and ask them to label 2-4 sentences as the ground-truth language descriptions. 

\begin{table}[htbp]
\centering
% \vspace{-15pt}
% \vskip -15 pt
%\begin{tabular}{c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\begin{tabular}{c|c|c|c|c|c|c|c|c}\hline
                           \#environments & \#clips & avg len & \#action types & \#object types & \#sentences & \#words & vocab & len (hrs) \\
\hline
10 &  1,035 & 31.3s & 157  & 38  & 3,610  & 77,762   & 6,910   & 8.99  \\
\hline    
\end{tabular}
% \vspace{10pt}
\vskip 10 pt
\caption{Statistics of our RCD dataset.}
\label{tab:dataset}
% \vspace{-20pt}
\vskip -20 pt
\end{table}

We summarize our dataset statistics in \autoref{tab:dataset}. In total, we collect 1,035 clips in 10 different in-door environments, including bedroom, kitchen, living room, lounge, office, etc. Each clip on average spans 31.3 seconds. The RCD dataset exhibits two types of diversity. 
{\it 1. Diversity of actions and objects:} Our RCD dataset contains 157 different actions and 38 different objects to interact with. The actions and objects are the same as the Charades dataset to ensure a similar action diversity. The same action is performed at different locations by different people, and different actions are performed at the same location. For example, all of the following actions are performed in the bathroom next to the sink: brushing teeth, washing hands, dressing, brushing hair, opening/closing a cabinet, putting something on a shelf, taking something off a shelf, washing something,  etc.
{\it  2. Diversity of environments:} Environments in our dataset differ in their floormap, position of furniture, and the viewpoint of the RF device. Further, each environment and all actions performed in that environment are included either in testing or training, but not both. 

%\red{Our RCD dataset contains 157 different actions and 38 different objects to interact with, in which the actions and objects are the same as that in the Charades dataset. Similar to the Charades dataset, our RCD dataset ensures diversity, that is, the same action can be performed at different locations by different people, and different actions can be performed at the same location by different people.}

% We record synchronized  RF signals and multi-view RGB videos while the volunteers perform the activities. We use a portable multi-camera system with 12 viewpoint to record the videos in case that some viewpoints may be occluded or the volunteers walk from one room to another room, where labeling based on a single view may get inaccurate sentence annotations. We provide each set of multi-view RGB videos to Amazon Mechanical Turk (AMT) workers and ask them to label 2-4 sentences as the ground-truth language descriptions. 

%We collect a new dataset which we call RF Captioning Dataset (RCD). Our dataset provides synchronized RF signals, multi-view videos, floormaps, as well as human-labeled captions to describe each event.  

% The RF signals are collected by an RF device, and multi-view RGB videos are collected by a portable multi-camera system with 12 viewpoints. floormaps are measured by a commercial laser meter. The synchronized radio signal and video has a maximum time difference of 10 ms. Figure (TODO) in Appendix shows the details of our system setup. 

%After collecting the multi-view video frames, we generate 3D skeletons by first running AlphaPose \cite{fang2017rmpe} on individual frames to generate 2D skeletons from each viewpoint, and then triangulate the 2D skeletons to get the 3D skeleton for each person. 

%In total, we collect 1,035 clips in 10 different in-door environments, including bedroom, kitchen, living room, lounge, office, etc. Each clip on average spans 31.3 seconds. 
%We use 685 clips from 7 environments for training and another 350 clips from 3 environments for testing. In the testing set, we have 175 samples in visible scenarios and another 175 samples in invisible scenarios, e.g. with occlusions or poor lighting conditions. Since it can be very hard for humans to label the event descriptions in these invisible scenarios, we ask the volunteers to perform the same series of activities twice under the visible and invisible environment (with light on and off, or with an occlusion in front of the RF device and cameras), respectively. Later we use the same ground truth language descriptions for the clips in the visible test set and the corresponding ones in the invisible test set. 
%\red{Environments in our dataset differ in their floormap, the position of furniture, and the viewpoint of the RF device. Further, each home/environment and the actions therein are included either in testing or training, with no overlap allowed. }

\vskip 0.06in\noindent
\textbf{(b)~Train-test Protocol:~~}To evaluate \name~under visible scenarios, we do a 10-fold cross-validation on our RCD Dataset. Each time 9 environments are used for training, and the other 1 environment is used for testing. We report the average performance of 10 experiments.
To show the performance of \name~under invisible scenarios, e.g., with occlusions or poor lighting conditions, we randomly choose 3 environments (with 175 clips) and collect corresponding clips under invisible conditions. Specifically, in these 3 environments, we ask the volunteers to perform the same series of activities twice under the visible and invisible conditions (with the light on and off, or with an occlusion in front of the RF device and cameras), respectively. Later we provide the same ground truth language descriptions for the clips under invisible conditions as the corresponding ones under visible conditions. During testing, clips under invisible scenarios in these 3 environments are used for testing, and clips in the other 7 environments are used to train the model.


% In total, we collect 1,035 clips in 10 different in-door environments, including bedroom, kitchen, living room, lounge, office, etc. For each clip, we randomly sample a caption from Charades dataset \cite{sigurdsson2016hollywood} and ask the volunteer to perform this caption. Then we label the clip with 2-4 ground truth language descriptions using the multi-view RGB videos. Each clip on average spans 31.3 seconds. Our RCD dataset provides 685 clips from 7 environments for training and 350 clips from 3 environments for testing. 

% In the testing set, we have 175 samples in visible scenario and 175 samples in invisible scenario, e.g. with occlusions or poor lighting conditions. Since it can be also hard for human to label events in invisible scenarios, we collect one visible sample and one invisible sample in pair. The subject first perform a series of activities (in visible environments). He is then asked to perform the same series of activities, but with light closed, or with an occlusion in front of the RF device and cameras. Later we use the same ground truth language description for the clips in visible test set and the corresponding ones in the invisible test set.

During training, we only use RGB videos from 3 cameras with good views instead of all 12 views in the multi-modal feature alignment between the video-captioning model and \name~model. Using multi-view videos will provide more training samples and help the feature space to be oblivious to the viewpoint. When testing the video-captioning model, we use the video from the master camera as it covers most of the scenes. The master camera is positioned atop of the RF device for a fair comparison.

%For video samples during training, 3 cameras with good views are used in the multi-modal feature alignment between the video-caption model and \name~model. This will provide more training samples and help the feature space to be oblivious to the viewpoint. For video samples during testing, we choose to use video frames from the master camera as it covers most of the scene. The master camera is built on top of the RF device for a fair comparison.

We leverage the Charades caption dataset \cite{sigurdsson2016hollywood,wang2018video} as the unpaired dataset to train the video-captioning model. This dataset provides captions for different in-door human activities. It contains 6,963 training videos, 500 validation videos, and 1,760 test videos. Each video clip is annotated with 2-5 language descriptions by AMT workers.

\vskip 0.06in\noindent
\textbf{(c)~Evaluation Metrics:~~}
We adopt 4 caption evaluation scores widely used in video-captioning: BLEU \cite{papineni2002bleu}, METEOR \cite{denkowski2014meteor}, ROUGE-L \cite{lin2004rouge} and CIDEr \cite{vedantam2015cider}. BLEU-$n$ analyzes the co-occurrences of $n$ words between the predicted and ground truth sentences. METEOR compares exact token matches, stemmed tokens, paraphrase matches, as well as semantically similar matches using WordNet synonyms. ROUGE-L measures the longest common subsequence of two sentences. CIDEr measures consensus in captions by performing a Term Frequency Inverse Document Frequency (TF-IDF) weighting for each $n$ words. According to \cite{sigurdsson2016hollywood}, CIDEr offers the highest resolution and most similarity with human judgment on the captioning task for in-home events. We compute these scores using the standard evaluation code provided by the Microsoft COCO Evaluation Server \cite{chen2015microsoft}. All results are obtained as an average of 5 trials. We denote B@n, M, R, C short for BLEU-n, METEOR, ROUGE-L, CIDEr.

\subsection{Quantitative Results}
We compare \name~with state-of-the-art video-captioning baselines~\cite{hu2019hierarchical,venugopalan2015sequence,yao2015describing,fakoor2016memory}. The video-based models are trained on RGB data from both the Charades and RCD training sets, and tested on the RGB data of the RCD test set. \name~is trained on RF and floormap data from the RCD training sets. It also uses the RGB data from Charades and RCD training sets in multi-modal feature alignment training. It is then tested on the RF and floormap data of the RCD test set.

The results on the left side of \autoref{tab:result-main} show that \name~achieves comparable performance to state-of-the-art video captioning baselines in visible scenarios. The right side of \autoref{tab:result-main} shows that \name~also generates accurate language descriptions when the environment is dark or with occlusion, where video-captioning fails completely. The little reduction in \name's performance from the visible scenario is likely due to that occlusions attenuate RF signals and therefore introduce more noise in the RF heatmaps.

\begin{table}[htbp]
\centering
% \vspace{-10pt}
\vskip -10 pt
%\begin{subtable}{.5\linewidth}
      \centering
      \begin{tabular}{l@{\hspace{0.2cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
      \hline
       \multirow{2}{*}{Methods}  & \multicolumn{7}{c}{Visible Scenario} & \multicolumn{7}{c}{Dark/Occlusion Scenario}\\ \cmidrule(lr){2-8} \cmidrule(lr){9-15} & B@1 & B@2 & B@3 & B@4 & M & R & C & B@1 & B@2 & B@3 & B@4 & M & R & C \\
      \hline\hline
       S2VT \cite{venugopalan2015sequence} & 57.3 & 40.4 &  27.2 & 19.3 & 19.8 & 27.3 & 18.9 &  -  & -  & -  & -  & -   & -  & – \\
       SA \cite{yao2015describing} & 56.8 & 39.2 & 26.7 & 19.0 & 18.1 & 25.9 & 22.1 &  -  & -  & -  & -  & -   & -  & –\\ 
       MAAM \cite{fakoor2016memory} & 57.8 & 41.9 & 28.2 & 19.3 & 20.7 & 27.1 & 21.2 &  -  & -  & -  & -  & -   & -  & – \\
       HTM \cite{hu2019hierarchical} & 61.3  & 44.6  &  32.2  & 22.1  & 21.3   & 28.3   & 26.5 &  -  & -  & -  & -  & -   & -  & –  \\

       HRL \cite{wang2018video} &  \textbf{62.5}  & 45.3  &  32.9  & \textbf{23.8}  & \textbf{21.7}   & 28.5   & \textbf{27.0} &  -  & -  & -  & -  & -   & -  & –  \\
      \hline
      \textbf{\name}  & 62.3  & \textbf{45.9}  &\textbf{33.9}  & 23.5  & 21.1   & \textbf{28.9}   & 26.7  & \textbf{61.5}  & \textbf{45.5}  & \textbf{33.1}  & \textbf{22.6}  & \textbf{21.1}   & \textbf{28.3}   & \textbf{25.9} \\
      \hline
\end{tabular}

%      \caption{Visible Scenario}
%    \end{subtable}%
%    \begin{subtable}{.5\linewidth}
%      \centering
%        \begin{tabular}{l |@{\hspace{0.05cm}} c @{\hspace{0.05cm}} c @{\hspace{0.05cm}}c @{\hspace{0.05cm}}c @{\hspace{0.05cm}}c @{\hspace{0.05cm}}c @{\hspace{0.05cm}}c}
%        \hline  
%         Method & B@1 & B@2 & B@3 & B@4 & M & R & C \\
%      \hline\hline
%        Video \cite{wang2018video} &  -  & -  & -  & -  & -   & -  & –  \\
%        \hline
%        \name  & \textbf{61.5}  & \textbf{45.5}  & \textbf{33.1}  & \textbf{22.6}  & \textbf{21.1}   & \textbf{28.3}   & \textbf{25.9}  \\
%        \hline     
%        \end{tabular}
%       \caption{Dark/Occlusion Scenario}
%    \end{subtable} 

\caption{\footnotesize{Quantitative results for \name~and video-based captioning models. All models are trained on Charades and RCD training set, and tested on the RCD test set. The left side of the Table shows the results under visible scenarios, and the right side of the Table shows the results under scenarios with occlusions or without light.}}
\label{tab:result-main}
% \vspace{-20pt}
\vskip -20 pt
\end{table}


%\subsection{Evaluation of Feature Alignment}
%In this section, we show the effectiveness of our feature alignment training. In \autoref{tab:result-sfcd} we show the results of \name~with or without applying the feature alignment training scheme. As shown in the table, for \name, aligning the features with videos to the unified space significantly improves the quality of its generated descriptions. This demonstrates that the multi-modal feature alignment training can help \name~utilize the knowledge of the video-captioning model learned from the large video-captioning dataset and generate accurate descriptions with training only on a rather small RCD dataset.
%
%\begin{table}[htbp]
%\centering
%\vspace{-5pt}
%\begin{tabular}{l |@{\hspace{0.1cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}
%\hline
%Method                 & B@1 & B@2 & B@3 & B@4 & M & R & C \\
%\hline\hline
%w/o align            & 52.5  & 38.0  & 25.7  & 18.5  & 16.6   & 23.1   & 20.3  \\
%\name  & \textbf{62.0}  & \textbf{46.2}  & \textbf{33.6}  & \textbf{23.6}  & \textbf{21.3}   & \textbf{28.7}   & \textbf{26.9}  \\
%\hline     
%\end{tabular}
%
%\begin{tabular}{c}
%(a) Visible Scenario
%\end{tabular}
%
%\begin{tabular}{l@{\hspace{0.21cm}}|@{\hspace{-0.12cm}} @{\hspace{0.27cm}} c @{\hspace{0.31cm}} c @{\hspace{0.31cm}}c @{\hspace{0.31cm}}c @{\hspace{0.27cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}
%\hline
%w/o align            & 52.3  & 37.4  & 25.5  & 17.6  & 16.5   & 23.1   & 20.0  \\
%\name  & \textbf{61.5}  & \textbf{45.5}  & \textbf{33.1}  & \textbf{22.6}  & \textbf{21.1}   & \textbf{28.3}   & \textbf{25.9}  \\
%\hline     
%\end{tabular}
%
%\begin{tabular}{c}
%(b) Dark/Occlusion Scenario
%\end{tabular}
%
%\caption{\footnotesize{Demonstration of the effectiveness of feature alignment. We show results of \name~on RCD test set with or without feature alignment training.}}
%\label{tab:result-sfcd}
%\vspace{-15pt}
%\end{table}



\vskip -0.2 in\noindent
\subsection{Ablation Study}
We conduct several ablation studies to demonstrate the necessity of each component in \name. All experiments here are evaluated on the visible test set of RCD.

\textbf{3D Skeleton vs. Locations:} One may wonder whether simply knowing the location of the person is enough to generate a good caption. This could happen if the RCD dataset has low diversity, i.e., each action is done in a specific location. This is however not the case in the RCD dataset, where each action is done in multiple locations, and each location may have different actions. To test this point empirically, we compare our model which extracts 3D skeletons from RF signals with a model that extracts only people locations from RF. We also compare with a model that extracts 2D skeletons with no locations (in this case the floormap's coordinate system is centered on the RF device).

\begin{table}[htbp]
\centering
% \vspace{-10pt}
\vskip -10 pt
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
Method                           & B@1 & B@2 & B@3 & B@4 & M & R & C \\
\hline

Locations                 & 52.0  & 37.4  & 24.3  & 17.2  & 15.7   & 22.1   & 19.1  \\
2D Skeletons              & 56.5  & 39.8  & 26.9  & 18.8  & 18.0   & 24.1   & 22.3  \\
3D Skeletons            & \textbf{62.3}  & \textbf{45.9}  & \textbf{33.9}  & \textbf{23.5}  & \textbf{21.1}   & \textbf{28.9}   & \textbf{26.7}  \\
\hline    
\end{tabular}
% \vspace{5pt}
\vskip 5 pt
\caption{\footnotesize{Comparison between using different human representations.}}
\label{tab:result-skl}
% \vspace{-20pt}
\vskip -20 pt
\end{table}

\autoref{tab:result-skl} shows that replacing \textit{3D skeletons} with  \textit{locations} or \textit{2D skeletons} yields poor performance.  This is because  \textit{locations} do not contain enough information of the actions performed by the person, and \textit{2D skeletons} do not contain information of the person's position with respect to the objects on the floormaps. These results show that: 1) our dataset is diverse and hence locations are not enough to generate correct captioning, and 2) our choice of representation, i.e., \textit{3D skeletons}, which combines information about both the people's locations and poses provides the right abstraction to learn meaningful features for proper captioning. 

\textbf{Person-Centric Floormap Representation:} 
In this work, we use a person-centric coordinate representation for the floormap and its objects, as described in \autoref{sec:floormap}. 
%What if we use a more direct representation, i.e. the top-down view of the floormap, encode object classes using different colors and represent the person's position as a dot (Appendix C)? 
What if we simply use the image of the floormap with the objects, and mark the map with the person's location at each time instance?  We compare this \textit{image-based floormap} representation to our person-centric representation in \autoref{tab:result-floormap}. We use ResNet-18 pre-trained on ImageNet to extract features from the floormap image. The result shows that the image representation of floormap can achieve better performance than not having the floormap, but still worse than our person-centric representation. This is because it is much harder for the network to interpret and extract features from an image representation, since the information is far less explicit than our person-centric coordinate-based representation. 

\begin{table}[h]
\centering
% \vspace{-10pt}
\vskip -10 pt
\begin{tabular}{@{\hspace{0.2cm}}l@{\hspace{0.2cm}} |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c@{\hspace{0.2cm}}}\hline
Method                           & B@1 & B@2 & B@3 & B@4 & M & R & C \\
\hline
w/o floormap & 56.3  & 40.8  & 27.7  & 18.5  & 18.1   & 24.0   & 22.1 \\
%\hline
image-based floormap & 60.1  & 43.9  & 31.5  & 21.6  & 20.1  & 26.7   & 24.4  \\
person-centric floormap& \textbf{62.3}  & \textbf{45.9}  & \textbf{33.9}  & \textbf{23.5}  & \textbf{21.1}   & \textbf{28.9}   & \textbf{26.7}  \\
person-centric floormap+noise& 61.6  & 45.8  & 33.7  & 23.4  & 21.0   & 28.7   & 26.5  \\

\hline     
\end{tabular}
% \vspace{5pt}
\vskip 5 pt
\caption{\footnotesize{Performance of \name~with or without using floormap, with different floormap representations, and with gaussian noise.}}
\label{tab:result-floormap}
\vskip -20 pt
% \vspace{-20pt}
\end{table}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\linewidth]{results}
\end{center}
% \vspace{-20pt}
\vskip -20 pt
\caption{\footnotesize{Examples from our RCD test set. Green words indicate actions. Blue words indicate objects included in floormap. Brown words indicate small objects not covered by floormap. Red words indicate the misprediction of small objects from \name. The first row shows \name~can generate accurate captions compared to the video-based captioning model under visible scenarios. The second row shows that \name~can still generate accurate captions when the video-based model does not work because of poor lighting conditions or occlusions. The third row shows the limitation of \name~that it may miss object color and detailed descriptions of small objects.}}\label{fig:results}
% \vspace{-15pt}
\vskip -15 pt
\end{figure*}

\textbf{Measurement Errors:} We analyze the influence of floormap measurement errors on our model's performance. We add a random gaussian noise with a 20cm standard deviation on location, 10cm on size and 30 degrees on object rotation. The results in the last row of \autoref{tab:result-floormap} show that the noise has very little effect on performance. This demonstrates that our model is robust to measurement errors.


\textbf{Feature Alignment}: Our feature alignment framework consists of two parts: the $L_2$-norm between paired dataset, and the discriminator between unpaired datasets. \autoref{tab:result-l2-dis}  quantifies the contribution of each of these alignment mechanisms to \name's performance. The results demonstrate that our multi-modal feature alignment training scheme helps \name~utilize the knowledge of the video-captioning model learned from the large video-captioning dataset to generate accurate descriptions, while training only on a rather small RCD dataset. We show a visualization of the features before and after alignment in the Appendix.

\begin{table}[h]
\centering
% \vspace{-10pt}
\vskip -10 pt
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
Method                           & B@1 & B@2 & B@3 & B@4 & M & R & C \\
\hline
w/o $L_2$     & 52.5  & 38.0  & 25.7  & 18.5  & 16.6   & 23.1   & 20.3  \\
w/o discrim & 59.4  & 44.1  & 31.4  & 21.0  & 19.8  & 26.3  & 24.6 \\
\hline
\name  & \textbf{62.3}  & \textbf{45.9}  & \textbf{33.9}  & \textbf{23.5}  & \textbf{21.1}   & \textbf{28.9}   & \textbf{26.7}  \\
\hline     
\end{tabular}
% \vspace{5pt}
\vskip 5 pt
\caption{\footnotesize{Performance of \name~network on RCD with or without $L_2$ loss and discriminator. Note that without adding the $L_2$ loss, \name~will not be affected by the video-captioning model. So if without the $L_2$ loss, then adding the discriminator loss on video-captioning model or not will not affect the \name's performance.}}
\label{tab:result-l2-dis}
% \vspace{-25pt}
\vskip -25 pt
\end{table}
%
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=1.0\linewidth]{distribution}
%\end{center}
%\caption{\footnotesize{Distribution of features extracted by \name~and video-captioning model. Left: without feature alignment. Middle: with $L_2$-norm, Right: with $L_2$-norm and discriminator.}}\label{fig:distribution}
%\end{figure}
%
%
%\textbf{Distribution Alignment}: to further illustrates the necessity and effectiveness of our feature alignment framework, we perform a visualization on the feature spaces we learned. In our feature alignment framework, there are in total three feature spaces: features extracted from RF+floormap on RCD, features extracted from videos on RCD, and features extracted from videos on Charades dataset. We visualize these three distributions using t-SNE to see the difference between them. 
%
%As shown in \autoref{fig:distribution}, without feature alignment (left), the two feature distributions extracted from the video-captioning network are close to each other while far away from the feature distribution of the \name. After applying the $L_2$-norm (middle), the features extracted from RF signals are aligned with the features extracted from the video on RCD, while the features extracted from Charades dataset are decoupled with those from RCD because only the features extracted from RCD are affected by the $L_2$-norm. In the third figure, we show that this decoupling can be solved by adding a discriminator between the two distributions.


%\subsection{Qualitative Result\protect\footnote{\red {We have a video demonstration on our  \href{http://rf-diary.csail.mit.edu}{website}.}}}
\subsection{Qualitative Result}
In \autoref{fig:results}, we show six examples from the RCD test set. The first row under each image is the caption generated by state of the art video-based captioning model \cite{wang2018video}, the second row is the caption generated by \name, and the third row is the ground truth caption labeled by a human. 

The result shows that \name~can generate accurate descriptions of the person's activities (green) and interaction with the surrounding environment (blue), and continue to work well even in the presence of occlusions (\autoref{fig:results} (c)), and poor lighting (\autoref{fig:results} (d)). Video-based captioning is limited by bad lighting, occlusions and the camera's field of view. So if the person exits the field of view, video captioning can miss some of the events (\autoref{fig:results} (e)).

Besides poor lighting conditions, occlusions and field of view, video-captioning is also faced with privacy problems. For example, in \autoref{fig:results} (b), the person just took a bath and is not well-dressed. The video will record this content which is quite privacy-invasive. However, RF signal can protect privacy since it is not interpretable by a human, and it does not contain detailed information because of the relatively low resolution.

%Video-caption can also fail when the environment is cluttered as shown in \autoref{fig:results} (a). This is because RGB videos, particularly in cluttered homes, contain a lot of extraneous background information, which makes the model extract features irrelevant to the foreground people. For example, in, video-caption generates incorrect description that the person is washing dishes because the person in the video is near a sink full of dishes. However, the person is actually in front of the stove. Our model uses 3D skeletons as intermediate representation and thus can harness the depth information from RF signals to localize the person, thus accurately recognizes that the person is cooking.

We also observe that \name\ has certain limitations. Since RF signals cannot capture details of objects such as color, texture, and shape, the model can mispredict those features. It can also mistake small objects. For example, in \autoref{fig:results} (e), the person is actually drinking orange juice, but \name\ predicts he is drinking water. Similarly, in \autoref{fig:results} (f), our model reports that the person is eating but cannot tell that he is eating a chocolate bar. The model also cannot distinguish the person's gender, so it always predicts ``he'' as shown in \autoref{fig:results} (e). 

\vskip -0.2 in\noindent
% \vspace{-5pt}
\vskip -5 pt
\subsection{Additional Notes on Privacy}
In comparison to images, RF signal is privacy-preserving because it is difficult to interpret by humans. However, one may also argue that since RF signals can track people though walls, they could create privacy concerns. This issue can be addressed through a challenge-response authentication protocol that prevent people from maliciously using RF signals to see areas that they are not authorized to access. More specifically, previous work~\cite{adib20143d} demonstrates that RF signals can sense human trajectories and locate them in space. Thus, whenever the user sets up the system to monitor an area, the system first challenges the user to execute certain moves (e.g., take two steps to the right, or move one meter forward), to ensure that the monitored person is the user. The system also asks the user to walk around the area to be monitored, and only monitors that area. Hence, the system would not monitor an area which the user does not have access to. 
% \vspace{-6pt}
\vskip -6 pt



==> arxiv eccv/source/intro-5.tex <==
\section{Introduction}
Captioning is an important task in computer vision and natural language processing; it typically generates language descriptions of visual inputs such as images or videos~\cite{venugopalan2015sequence,yao2015describing,fakoor2016memory,baraldi2017hierarchical,yu2016videornn,pan2016hierarchical,song2017hierarchical,wu2018interpretable,hu2019hierarchical,ranzato2015sequence,pasunuru2017reinforced,wang2018video}. This paper focuses on {\it in-home daily-life captioning}, that is, creating a system that observes people at home, and automatically generates a transcript of their everyday life. Such a system would help older people to age-in-place. Older people may have memory problems and some of them suffer from Alzheimer's. They may forget whether they took their medications, brushed their teeth, slept enough, woke up at night, ate their meals, etc. Daily life captioning enables a family caregiver, e.g., a daughter or son, to receive text updates about their parent's daily life, allowing them to care for mom or dad even if they live away, and providing them peace of mind about the wellness and safety of their elderly parents. More generally, daily-life captioning can help people track and analyze their habits and routine at home, which can empower them to change bad habits and improve their life-style. 

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{teaser}
\end{center}
\vskip -15 pt
\caption{\footnotesize{Event descriptions generated from videos and RF+Floormap. The description generated from video shows its vulnerability to poor lighting and confusing images, while \name\ is robust to both. The visualization of floormap shown here is for illustration.  The representation used by our model is person-centric and is described in detail in section~\ref{sec:floormap}.
%The red dotted line and the red dot on the floormap illustrate the person's path and location, respectively.
}}\label{fig:teaser}
\vskip -15 pt
\end{figure*}


But how do we caption people's daily life? One option would be to deploy cameras at home, and run existing video-captioning models on the recorded videos. However, most people would have privacy concerns about deploying cameras at home, particularly in the bedroom and bathroom. Also, a single camera usually has a limited field of view; thus, users would need to deploy multiple cameras covering different rooms, which would introduce a significant overhead. Moreover, cameras do not work well in dark settings and occlusions, which are common scenarios at home. 

To address these limitations, we propose to use radio frequency (RF) signals for daily-life captioning. RF signals are more privacy-preserving than cameras since they are difficult to interpret by humans. Signals from a single RF device can traverse walls and occlusions and cover most of the home. Also, RF signals work in both bright and dark settings without performance degradation. Furthermore, the literature has shown that one can analyze the radio signals that bounce off people's bodies to capture people's movements~\cite{adib20143d,adib2013see}, and track their 3D skeletons~\cite{zhao2018rf}. 


%Furthermore, RF signals reflect off the human body, and recent work has shown that those reflections can be processed by a neural network to infer the 3D pose of people in the environment, and how they move~\cite{zhao2018rf}.  

However, using RF signals also introduces new challenges, as described below: 

% While RF-based captioning has many advantages, it also introduces new challenges as follows:
\begin{Itemize}
\item {\bf Missing objects information:} RF signals do not have enough information to differentiate objects, since many objects are partially or fully transparent to radio signals. Their wavelength is on the order of a few centimeters, whereas the wavelength of visible light is hundreds nanometer~\cite{barbrow1964international}. Thus, it is also hard to capture the exact shape of objects using RF signals. 
\item {\bf Limited training data:} Currently, there is no training dataset that contains RF signals from people's homes with the corresponding captions. Training a captioning system typically requires tens of thousands of labeled examples. However, collecting a new large captioning dataset with RF in people's homes would be a daunting task.
\end{Itemize}


In this paper, we develop \name, an RF-based in-home daily-life captioning model that addresses both challenges. To capture objects information, besides RF signals, \name\ also takes as input the home floormap marked with the size and location of static objects like bed, sofa, TV, fridge, etc. Floormaps provide information about the surrounding environment, thus enabling the model to infer human interactions with objects. Moreover, floormaps are easy to measure with a cheap laser-meter in less than 10 minutes (Section~\ref{sec:floormap}). Once measured, the floormap remains unchanged for potentially years, and can be used for all future daily-life captioning from that home.

%RF signals embed information about 3D space, and hence when combined with a floormap, \name\ can extract information about people's position with respect to the surrounding objects, which is informative for inferring interaction with objects. Second, floormaps are easy to measure in a few minutes, with a cheap laser-meter (see section 4.2). %Further, the model needs only approximate measurements and does not need exact shape or size of objects. Third, 
 

\name\ proposes an effective representation to integrate the information in the floormap with that in RF signals. It encodes the floormap from the perspective of the person in the scene. It first extracts the 3D human skeletons from RF signals as in~\cite{zhao2018rf} and then at each time step, it shifts the reference system of floormap to the location of the extracted skeleton, and encodes the location and orientation of each object with respect to the person in the scene. This representation allows the model, at each time step, to focus on various objects depending on their proximity to the person.

To deal with the limited availability of training data, we propose a multi-modal feature alignment training scheme to leverage existing video-captioning datasets for training \name. To transfer visual knowledge of event captioning to our model, we align the features generated from \name\ to the same space of features extracted from a video-captioning model trained on existing large video-captioning datasets. Once the features are aligned, we use a language model to generate text descriptions.

\autoref{fig:teaser} shows the performance of our model in two scenarios. In the first scenario, a person wakes up from bed, puts on his shoes and clothes, and goes to his desk to work on his laptop. \name\ generates a correct description of the events, while video-captioning fails due to poor lighting conditions. The second scenario shows a person cooking on the stove. Video-captioning confuses the person's activity as washing dishes because, in the camera view, the person looks as if he were near a sink full of dishes. In contrast, \name\ generates a correct caption because it can extract 3D information from RF signals, and hence can tell that the person is near the stove not the sink. 
 

To evaluate \name, we collect a captioning dataset of RF signals and floormaps, as well as the synchronized RGB videos.
Our experimental results demonstrate that: 1) \name~can obtain comparable results to video-captioning in visible scenarios. Specifically, on our test set, \name\ achieves 41.5 average BLEU and 26.7 CIDEr, while RGB-based video-captioning achieves 41.1 average BLEU and 27.0 CIDEr. 2) \name~continues to work effectively in dark and occluded conditions, where video-captioning methods fail. 3) Finally, our ablation study shows that the integration of the floormaps into the model and the multi-modal feature alignment both contribute significantly to improving performance. 

Finally, we summarize our contributions as follows:
\begin{Itemize}
    \item We are the first to caption people's daily-life at home, in the presence of bad lighting and occlusions. 
    \item We also introduce new modalities: the combination of RF and floormap, as well as new representations for both modalities that better tie them together.      
    \item We further introduce a multi-modal feature alignment training strategy for knowledge transfer from a video-captioning model to \name. 
    \item We evaluate our RF-based model and compare its performance to past work on video-captioning.  Our results provide new insights into the strengths and weaknesses of these two types of inputs. 
\end{Itemize}


==> arxiv eccv/source/method-2.tex <==
% \vspace{0pt}
\section{\name}
\label{sec:method}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{model}
\end{center}
% \vspace{-5pt}
\vskip -5 pt
%\caption{\footnotesize{Model architecture. In the left yellow box, \name\ extract features from RF signals $\textbf{R}^P$ and floormaps $\textbf{F}^P$ and then combine them to a unified human-environment feature $\textbf{u}^{P}$. In the right blue box, it extracts features from both paired and unpaired videos $\textbf{X}^P, \textbf{X}^U$ and get $\textbf{v}_n^{P}, \textbf{v}_n^{U}$. The features are then taken by the language generation network (green box) and generate captions. During training, \name~applies an $L_2$-loss ($\mathcal{L}_{pair}$) between $\textbf{v}_n^P$ and $\textbf{u}^P$ extracted from paired video and RF-Floormap data; a discriminator loss ($\mathcal{L}_{unpair}$) between $\textbf{v}_n^{P}, \textbf{v}_n^{U}$ extracted from paired and unpaired video data; and the caption loss $\mathcal{L}_{caption}$. During testing, it takes only the RF+Floormap without video as input and generates captions.}}\label{fig:method}
%\caption{\footnotesize{Model architecture. It contains four parts: RF+Floormap feature extraction (the left yellow box), video feature extraction (the right blue box), unified embedding space (the center grey box), and language generation network (the bottom green box). In the left yellow box, \name\ extracts features from RF signals $\textbf{R}^P$ and floormaps $\textbf{F}^P$ and combines them into a unified human-environment feature map $\textbf{u}^{P}$. In the right blue box, \name\ extracts features from both paired videos $\textbf{X}^P $ (synchronized videos with RF+Floormap) and unpaired videos $\textbf{X}^U$ (an existing video captioning dataset), and gets the video representation $\textbf{v}_n^{P}, \textbf{v}_n^{U}$. The features $ \textbf{u}^{P} $, $\textbf{v}_n^{P} $, $\textbf{v}_n^{U}$ are then taken by the language generation network (the bottom green box) to generate captions. During training, besides the caption loss $\mathcal{L}_{cap}$, \name\ adds additional losses to map the features in different modalities into a unified embedding space (the center grey box). \name\ applies an $L_2$-loss ($\mathcal{L}_{pair}$) between $\textbf{v}_n^P$ and $\textbf{u}^P$ extracted from paired video and RF+Floormap data, and a discriminator loss ($\mathcal{L}_{unpair}$) via adversarial training between $\textbf{v}_n^{P}, \textbf{v}_n^{U}$ extracted from paired and unpaired video data. During testing, \name\ takes only the RF+Floormap without videos as input and generates captions.}}
\caption{\footnotesize{Model architecture. It contains four parts: RF+Floormap feature extraction (the left yellow box), video feature extraction (the right blue box), unified embedding space for feature alignment (the center grey box), and language generation network (the bottom green box). \name\ extracts features from RF signals and floormaps and combines them into a unified human-environment feature map. The features are then taken by the language generation network to generate captions. \name\ also extracts features from both paired videos (synchronized videos with RF+Floormap) and unpaired videos (an existing video captioning dataset), and gets the video representation. These features are used to distill knowledge from existing video dataset to \name. During training, \name\ uses the caption loss and the feature alignment loss to train the network. During testing, \name\ takes only the RF+Floormap without videos as input and generates captions.}}
\label{fig:method}
% \vspace{-15pt}
\vskip -15 pt
\end{figure*}


% \vspace{-5pt}
\vskip -5 pt
\name\ generates event captions using RF signals and floormaps. As shown in \autoref{fig:method}, our model first performs feature extraction from RF signals and floormaps, then combine them into a unified feature (the left yellow box). The combined feature is taken by a language generation network to generate captions (the bottom green box). Below, we describe the model in detail. We also provide implementation details in Appendix A.

%\name\ generates event captions based on RF signals and floormaps. As shown in \autoref{fig:method}, our model first performs feature extraction from RF signals and floormaps (the left yellow box) and then uses a sequence-to-sequence encoder-decoder model to generate captions (the bottom green box). Below, we describe the model in detail.

\subsection{RF Signal Encoding}
RF signals have properties totally different from visible light, which are usually not interpretable by human. Therefore, it can be hard to directly generate captions from RF signals. However, recent works demonstrate that it is possible to generate accurate human skeletons from radio signals \cite{zhao2018rf}, and that the human skeleton is a succinct yet informative representation for human behavior analysis \cite{li2018co,du2015skeleton}. In this work, we first generate 3D human skeletons from RF signals, then extract the feature representations of the 3D skeletons.

Thus, the first stage in \name\ is a skeleton generator network, which has an 
architecture similar to the one in \cite{zhao2018rf}, with 90-frame RF heatmaps (3 seconds) as input; we refer to these 90 frames as an RF segment.  The skeleton generator first extracts information from the RF segment with a feature extraction network (12-layer ResNet). This is  followed by a region proposal network (6-layer ResNet) to generate region proposals for potential human bounding boxes and a pose estimation network (2-layer ResNet) to generate the final 3D skeleton estimations based on the feature maps and the proposals.  Note that these are dynamic skeletons similar to skeletons extracted from video segment. 

After we obtain the 3D skeletons from RF signals, we extract the feature representation through a skeleton encoder from each skeleton segment $ \textbf{S} $. The skeleton encoder is a Hierarchical Co-occurrence Network (HCN) \cite{li2018co}, which is a CNN-based network architecture for skeleton-based action recognition. We use the features from the last convolutional layer of HCN, denoted as $ \textbf{u}_{rf} $, as the encoded features for RF signals. 






\begin{figure}[htbp]
\begin{center}
%\vspace{-5pt}
\includegraphics[width=0.81\linewidth]{floormap}
\end{center}
\caption{\footnotesize{Illustration of floormap representation. Noted that this figure is not the input to our model but only a visualization. Red dotted line in the apartment denotes the moving path of a person from time $ t_{1} $ to $ t_{5}$. Green axes X-Y centered at the person illustrate our person-centric coordinate system, where the origin of the coordinate system is changed through time along with people's location. Under this person-centric coordinate system, at $ t^{th} $ time step, we describe each object using a 5-element tuple: (length $L$, width $W$, center coordinates $x(t), y(t)$, and rotation $\theta$), as exemplified using the \textbf{Table} in the figure.}}
%\caption{\footnotesize{Illustration of floormap representation. Noted that this figure is not the input to our model but only a visualization. The figure shows a floormap of an apartment. Red dotted line denotes the moving path of a person from time $ t_{1} $ to $ t_{5}$. Green axes illustrate our dynamic coordinate system, where the origin of the system is set to the center of the person. We describe each object using a 5-element tuple: (width $W$, height $H$, center coordinates $x(t), y(t)$, and rotation $\theta$), as exemplified using the \textit{Desk} in the figure.}}
\label{fig:floormap}
% \vspace{-15pt}
\vskip -15 pt
\end{figure}

%\vspace{-10pt}
\vskip -0.2 in\noindent
\subsection{Floormap Encoding}
\label{sec:floormap}

Many objects are transparent or semi-transparent to RF signals and act in a manner similar to air~\cite{adib2013see}. Even objects that are not transparent to RF signals, they can be partially invisible; this is because they can deflect the incident RF signal away from the emitting radio, preventing the radio from sensing them~\cite{zhao2018through,zhao2018rf}. 
Thus, to allow the model to understand interactions with objects, we must provide additional information about the surrounding environment. But we do not need to have every aspect of the home environment since most of the background information, e.g. the color or the texture of furniture, is irrelevant to captioning daily life. Therefore, we represent the in-home environment using the locations and sizes of objects -- the floormap. The floormap is easily measured with a laser meter. Once measured, the floormap tends to remain valid for a long time.  In our model, we only consider static objects relevant to people's in-home activities, e,g., bed, sofa, stove, or TV. To demonstrate the ease of collecting such measurements, we have asked 5 volunteers to measure the floormap for each of our test environments. The average time to measure one environment is about 7 mins.
 
Let $M$ be the number of objects, $N$ be the maximum number of instances of an object, then the floormap can be represented by a tensor $f\in\mathbb{R}^{M\times N\times O}$, where $O$ denotes the dimension for the location and size of each object, which is typically 5, i.e., length $L$, width $W$, the coordinate of the center $x(t),y(t)$, and its rotation $\theta$. 
%as shown with the example of a desk in figure \ref{fig:floormap}, 
%In our model, we only consider relatively static objects which are relevant to people's in-home activities and can be easily measured with a laser meter. The object list of floor-map we use is: cabinet, table, desk, bed, wardrobe, shelf, drawer, stove, fridge, sink, sofa, television, door, window, air conditioner, bathtub, dishwasher, oven, bedside table. To demonstrate the ease of collecting such measurements, we asked 5 volunteers to measure the floor-map for each environment in our dataset. The average time to measure one environment is 426 sec. Once a floor-map for a room is measured, it can remain unchanged for a long time. 


Since people are more likely to interact with objects close to them,  we set the origin point of the floormap reference system to the location of the 3D skeleton extracted from RF. Specifically, we use a person-centric coordinate system as shown in the green $X$-$Y$ coordinates in \autoref{fig:floormap}. A person is moving around at home in a red-dotted path from time $ t_{1} $ to $ t_{5}$. At each time step $t_{i} $, we set the origin of the 3D coordinate system to be the center of the 3D human skeleton and the $X$-$Y$ plane to be parallel to the floor plane. The orientation of the $X$-axis is parallel to the RF device and $Y$-axis is perpendicular to the device. Each object is then projected onto the $X$-$Y$ plane. For example, at time $ t_{i} $, the center coordinates of the \textbf{Table} is $ (x_{1}(t_{i}), y_{1}(t_{i}))$, while its width, length and rotation $ (L_{1}, W_{1}, \theta_{1}) $ are independent of time. The floormap at time $ t_{i} $ is thus generated by describing each object $ k $ using a 5-element tuple: $(L_{k}, W_{k}, x_{k}({t_{i}}), y_{k}({t_{i}}),\theta_{k}) $, as shown in the left yellow box in Figure~\ref{fig:method}. In this way, each object's location is encoded w.r.t. the person's location, allowing our model to pay different attention to objects depending on their proximity to the person at that time instance. 

To extract features of the floormaps $ \textbf{F} $, we use a floormap encoder which is a two-layer fully-connected network which generates the encoded features for floormaps $ \textbf{u}_{flr} $. 

Using the encoded RF signal features $ \textbf{u}_{rf} $ and floormap features $ \textbf{u}_{flr} $, we generate a unified human-environment feature: $$ \textbf{u} = \psi(\textbf{u}_{rf} \oplus \textbf{u}_{flr}),$$ 
where $\oplus$ denotes the concatenation of vectors, and $\psi$ denotes an encoder to map the concatenated features to a joint embedding space. Here we use another two-layer fully-connected sub-network for $\psi$.

\subsection{Caption Generation}
To generate language descriptions based on the extracted features, we use an attention-based sequence-to-sequence LSTM model similar to the one in \cite{venugopalan2015sequence,wang2018video}. During the encoding stage, given the unified human-environment feature $\textbf{u}=\{u_t\}_{1}^{T} $ with time dimension $ T $, the encoder LSTM operates on its time dimension to generate hidden states $\{h_t\}_{1}^{T}$ and outputs $\{o_t\}_{1}^{T}$. During the decoding stage, the decoder LSTM uses $h_T$ as an initialization for hidden states and take inputs of previous ground-truth words with an attention module related to  $ \{u_t\}_{1}^{T} $, to output language sequence with $m$ words $\{w_1, w_2, ..., w_m\}$. The event captioning loss $\mathcal{L}_{cap}(\textbf{u})$ is then given by a negative-log-likelihood loss between the generated and the ground truth caption similar to \cite{venugopalan2015sequence,wang2018video}.

\section{Multi-Modal Feature Alignment Training}
%\section{Teacher-Student Network Knowledge Distillation}
Training \name\ requires a large labeled RF captioning dataset. Collecting such a dataset would be a daunting task. To make use of the existing large video-captioning dataset (e.g., Charades), we use a multi-model feature alignment strategy in the training process to transfer knowledge from video-captioning to  \name. However, RGB videos from Charades and RF signals have totally different distributions both in terms of semantics and modality. To mitigate the gap between them and make the knowledge distillation possible, we collect a small dataset where we record synchronized videos and RF from people performing activities at home. We also collect the floormaps and provide the corresponding natural language descriptions (for dataset details see section~\ref{sec:dataset}(a)). The videos in the small dataset are called paired videos, since they are in the same semantic space as their corresponding RF signal, while the videos in large existing datasets are unpaired videos with the RF signals. Both the paired and unpaired videos are in the same modality. Since the paired videos share the same semantics with the RF data, and the same modality with the unpaired videos, they can work as a bridge between video-captioning and \name, and distill knowledge from the video data to RF data. 

%The objective of the feature alignment training is to allow our RF-based captioning model to leverage knowledge from those RGB-based video captioning datasets. We distinguish between two types of datasets: unpaired datasets, and paired datasets. Unpaired datasets are those large datasets (e.g., Charades) that only contain RGB-based videos and their corresponding natural language descriptions. Paired datasets refer to datasets with synchronized RGB videos, RF signals and corresponding floor-maps. Unfortunately there is no existing paired dataset, so we collect a small dataset where we record synchronized videos and RF on people performing daily activities in their homes and provide natural language description of each paired example (for dataset details see section~\ref{sec:dataset}(a)). Our training scheme learns from both types of datasets.

Our multi-modal feature alignment training scheme operates by aligning the features from RF+Floormaps and those from RGB videos. During training, our model extracts features from not only RF+Floormaps, but also paired and unpaired RGB videos, as shown in Figure~\ref{fig:method} (the right blue box). Besides the captioning losses, we add additional paired-alignment loss between paired videos and RF+Floormaps and unpaired-alignment loss between paired and unpaired videos. This ensures features from the two modalities are mapped
to a unified embedding space (the center grey box). Below, we describe the video encoder and the feature alignment method in detail.

%The alignment contains two parts: alignment of RF+Floormaps and paired videos in the same semantic space using the $L_2$-norm (the blue dotted ellipse); and alignment of paired videos and unpaired videos in the same feature distribution (the red dotted square). For paired data, we perform sample-based alignment to align the features from the RF+Floormaps and that from the corresponding RGB video using the $L_2$-norm. For unpaired data, we perform alignment on the distribution of the features of paired and unpaired videos via adversarial training. During testing, the RF-based network operates on its own and generate accurate captions without input any paired or unpaired videos. Below, we describe the video encoder and the feature alignment methods in detail. 

%Our multi-modal feature alignment training scheme operates by aligning the features from RF+Floor-maps and those from RGB videos. During training, our model extracts features from not only RF+Floor-maps, but also RGB videos (the blue box). Our model adds additional losses to ensures that features from the two modalities are aligned and leverage this property to transfer the knowledge learned from large RGB-based video captioning datasets to the RF-based network. For paired data, we perform sample-based alignment, where the features from the RF and floor-maps are aligned with the features from the corresponding RGB video using the $L_2$-norm. For unpaired data, there is no correspondence between an RGB video and a particular skeleton clip. Therefore, we perform distribution-based alignment using a discriminator. During testing, the RF-based network operates on its own and generate accurate captions without input videos. Below, we describe the video encoder and the feature alignment methods in detail. 

\subsection{Video Encoding}
\label{sec:video_encoding}
We use the I3D model~\cite{carreira2017quo} pre-trained on Kinetics dataset to extract the video features. For each 64-frame video segment, we extract the Mixed\_5c features from I3D model, denoted as $ v_{m} $. We then apply a spatial average pooling on top of the Mixed\_5c feature and get the spatial pooled video-segment feature $ v_{n}$. For a video containing $ T $ non-overlapping video-segment, its Mixed\_5c features and the spatial-pooled features are denoted as $ \textbf{v}_{m} = \{v_{m}(t)\}_{1}^{T}$ and $ \textbf{v}_{n} = \{v_{n}(t)\}_{1}^{T}$. Therefore, the extracted features of paired videos $ \textbf{X}^{P} $ and unpaired videos $ \textbf{X}^{U} $ are denoted as $ \textbf{v}_{m}^{P} $, $ \textbf{v}_{n}^{P} $ and $ \textbf{v}_{m}^{U} $, $ \textbf{v}_{n}^{U} $. We use the spatial-pooled features to generate captions through the language generation model. The corresponding captioning loss is $\mathcal{L}_{cap}(\textbf{v}_{n}^{P})$ and $\mathcal{L}_{cap}(\textbf{v}_{n}^{U})$. 

%We use the I3D model~\cite{carreira2017quo} pre-trained on Kinetics dataset to extract the video representations for both the paired videos $ \textbf{X}^{P} $ and unpaired videos $ \textbf{X}^{U} $. For each 64-frame video-segment in a paired or unpaired video, we extract the Mixed\_5c features from I3D model, denoted as $ v_{m}^{P} $ or $ v_{m}^{U} $. We then apply a spatial average pooling on top of the Mixed\_5c features and get the spatial pooled video-clip feature $ v_{n} ^{P}$ or $ v_{n}^{U} $. For a video containing $ T $ non-overlap video-clips, its Mixed\_5c features and the spatial-pooled features are denoted as $ \textbf{v}_{m} = \{v_{m}(t)\}_{1}^{T}$ and $ \textbf{v}_{n} = \{v_{n}(t)\}_{1}^{T}$. 

%The video encoder takes the raw video frames and generates feature maps. We choose to use the i3D model \cite{carreira2017quo} to encode the video frames. We apply an average pooling on top of the Mixed\_5c feature and use them as our video features $V$.

\subsection{Alignment of Paired Data}
\label{sec:pair}
%To transfer the knowledge from video-based network to RF-based network, we operate feature alignment on RF+Floor-maps and their corresponding paired videos. 
Since the synchronized video and RF+Floormap correspond to the exact same event, we use $L_2$ loss to align the features from paired video $ \textbf{v}_{n}^{P} $ in Sec~\ref{sec:video_encoding} and RF+Floormap $ \textbf{u}^{P} $ in Sec~\ref{sec:floormap} (we deonte a $ P $ here to indicate the paired data) to be consistent with each other in a unified embedding space, i.e., the paired data alignment loss $ \mathcal{L}_{pair}(\textbf{u}^{P}, \textbf{v}_{n}^{P}) = \left\lVert \textbf{u}^{P} - \textbf{v}_{n}^{P} \right\rVert_{2} $. 
%During training, this loss is combined with the \name\ captioning loss $\mathcal{L}_{cap}(\textbf{u}^{P})$ and paired video-captioning loss $ \mathcal{L}_{cap}(\textbf{v}_{n}^{P}) $ for back-propagation.

%To transfer the knowledge from video-based network to RF-based network, we operate feature alignment on paired video-RF-floormap data: the video, RF and floor-maps correspond to the exact same event. 
%We use an $L_2$ loss to align the features from synchronized video and RF+Floor-map to be consistent with each other in a unified embedding space. During training on paired data, this loss is combined with the caption loss $L_{caption}$ for back-propagation.

%Denoting the features from video frames by $V$ and those from the RF+Floor-maps by $U$, we define the feature alignment loss on paired data as:
%$$\mathcal{L}_{align}=\left\lVert V - U \right\rVert_2,$$
%which is an $L_2$ loss to align the features from videos and skeletons to be consistent with each other in a unified embedding space. During training on paired data, this loss is combined with the caption loss $L_{caption}$ for back-propagation.

\subsection{Alignment of Unpaired Data}
Existing large video-captioning datasets have neither synchronized RF signal nor the corresponding floormaps, so we cannot use the $L_2$-norm for alignment. Since we collect a small paired dataset, we can first train a video-captioning model on both paired and unpaired datasets, and then use the paired dataset to transfer knowledge to \name. However, the problem is that since the paired feature alignment is only applied on the paired dataset, the video-captioning model may overfit to the paired dataset and cause inconsistency between the distribution of features from paired and unpaired datasets.
%Since the paired videos in our collected dataset share the same semantic with the RF+Floor-maps data and share a the same modality with the unpaired large-scale videos. It can be considered to be a bridge between the unpaired videos and the RF+Floor-map data. As we have aligned the paired videos and RF+Floor-maps into a unified embedding space in Sec.~\ref{sec:pair}, we then only need to align the paired videos and unpaired videos into a unified modality distribution. 
To solve this problem, we align the paired and unpaired datasets by making the two feature distributions similar. We achieve this goal by applying discriminators on different layers of video features that enforces the video encoder to generate indistinguishable features given $ \textbf{X}^{P}$ and  $ \textbf{X}^{U} $. Specifically, we use two different layers of video features, i.e., $ \textbf{v}_{m} $ and $ \textbf{v}_{n} $ in Sec~\ref{sec:video_encoding}, to calculate the discriminator losses $\mathcal{L}_{unpair}(\textbf{v}_{m}^{P}, \textbf{v}_{m}^{U}) $ and $ \mathcal{L}_{unpair}(\textbf{v}_{n}^{P}, \textbf{v}_{n}^{U}) $. Since features from the paired videos are also aligned with the RF+Floormap features, this strategy effectively aligns the feature distribution of the unpaired video with the feature distribution of RF+Floormaps. The total loss of training process is shown as below:
% \vspace{-7pt}
\vskip -7 pt
\begin{eqnarray*}
\mathcal{L} &=& \mathcal{L}_{cap}(\textbf{u}^{P}) + \mathcal{L}_{cap}(\textbf{v}_{n}^{P}) + \mathcal{L}_{cap}(\textbf{v}_{n}^{U})  \\
&&  + \mathcal{L}_{pair}(\textbf{u}^{P}, \textbf{v}_{n}^{P})  \\
&&  + \mathcal{L}_{unpair}(\textbf{v}_{n}^{P}, \textbf{v}_{n}^{U}) + \mathcal{L}_{unpair}(\textbf{v}_{m}^{P}, \textbf{v}_{m}^{U}).
\end{eqnarray*}
%\vspace{-8pt}

%Existing video-captioning datasets have neither synchronized RF signal nor the corresponding floor-maps. So how can we leverage this large dataset for improving our model? We cannot use the $L_2$-norm for alignment as there is no paired examples. However, since we collect a small paired dataset, we can train the same RGB-based model and the language model on both paired and unpaired datasets, and use the paired dataset to transfer the knowledge of RGB-based model to the RF-based model. But there is still a problem that since the feature alignment loss is only on the paired dataset, the RGB-based model can overfit to the paired dataset and cause an inconsistency between the distribution of features from paired and unpaired datasets.

%To solve this problem, we further align the feature distribution of the RGB videos from paired and unpaired datasets using a discriminator. Since features from the paired RGB videos are also aligned with the RF+Floor-map features (using $L_2$-norm), this effectively aligns the feature distribution of the unpaired video with the feature distribution from the RF+Floor-maps using RGB-video from paired dataset as the bridge. The discriminator loss is also combined with the caption loss $L_{caption}$ on both paired and unpaired datasets during training.

%Specifically, we denote videos with synchronized skeletons as $x^s$ and those without skeletons as $x^c$. Let $v_L^s$ be the feature from the last conv layer of the video encoder on a source video $x^s$, and $v_L^c$ be the corresponding feature on video $x^c$. Denoting $Pr$ as the distribution of features, our goal is to make the two feature distributions similar, i.e. $Pr(v_L^s) \approx Pr(v_L^c)$. We achieve this goal by applying a discriminator (as shown in the blue box in \autoref{fig:method}) between $v_L^s$ and $v_L^c$ which enforces the video encoder to generate indistinguishable features given $x^s$ and $x^c$. The discriminator loss is then combined with the caption loss $L_{caption}$ for backpropagation. In this way, latent features from videos without synchronized skeletons are also forced to be in the unified space, and we can train the framework jointly using both Charades and our dataset.

==> arxiv eccv/source/related-2.tex <==
\section{Related Work}
% \vspace{-5pt}
\vskip -5 pt
\noindent\vskip 0.06in {\bf (a)~RGB-Based Video Captioning.}
Early works on video-captioning are direct extensions of image captioning. They pool features from individual frames across time, and apply image captioning models to video-captioning~\cite{venugopalan2015translating}. Such models cannot capture temporal dependencies in videos. Recent approaches, e.g., sequence-to-sequence video-to-text (S2VT), address this limitation by adopting recurrent neural networks (RNNs)~\cite{venugopalan2015sequence}. In particular, S2VT customizes LSTM for video-captioning and generates natural language descriptions using an encoder-decoder architecture. 
Follow-up papers improve this model by introducing an attention mechanism \cite{yao2015describing,fakoor2016memory,long2018video}, leveraging hierarchical architectures \cite{baraldi2017hierarchical,yu2016videornn,hu2019hierarchical,song2017hierarchical,gan2017stylenet,gan2017semantic}, 
or proposing new ways to improve feature extraction from video inputs, such as C3D features \cite{yao2015describing} or trajectories \cite{wu2018interpretable}. There have also been attempts to use reinforcement learning to generate descriptions from videos \cite{ranzato2015sequence,pasunuru2017reinforced,wang2018video}, in which they use the REINFORCE algorithm to optimize captioning scores.

\noindent\vskip 0.06in {\bf (b)~Human Behavior Analysis with Wireless Signals.} 
Recently, there has been a significant interest in analyzing the radio signals that bounce off people's bodies to understand human movements and behavior. Past papers have used radio signals to track a person's location \cite{adib20143d}, extract 3D skeletons of nearby people \cite{zhao2018rf}, or do action classification \cite{li2019making}. %However, all those approaches only analyze people's own behavior, and none of them have considered human interactions with the surrounding environment. 
To the best of our knowledge, we are the first to generate natural language descriptions of continuous and complex in-home activities using RF signals. Moreover, we introduce a new combined modality based on RF+Floormap and a novel representation that highlights the interaction between these two modalities, as well as a multi-modal feature alignment training scheme to allow RF-based captioning to learn from existing video captioning datasets. 

%\noindent\vskip 0.06in {\bf (c)~ Anonymization or Thermal Cameras for In-Home Monitoring.} 
% One may wonder whether the use of thermal cameras or anonymized RGB videos could address the problem, and eliminate the need for RF.  While such approaches can address one aspect of the problem (improving privacy or dealing with dark settings), RF signals can deal with both privacy issues and bad lighting. Furthermore, they work through walls and occlusions, which are common scenarios at home, where there are multiple rooms and occlusions from walls and furniture. No thermal or anonymized RGB cameras work through walls and occlusions~\cite{titman2001applications}.

==> arxiv eccv/source/rf.tex <==
\section{RF Signal Preliminary}

In this work, we use a radio commonly used in prior works on RF-based human sensing~\cite{zhao2018rf,hsu2017zero,hsu2019enabling,lien2016soli,peng2016fmcw,tian2018rf,chetty2017low,zhao2016emotion,zhao2019through,zhang2018latern,zhao2017learning,fan2020learning,hsu2017extracting}. The radio has two antenna arrays organized vertically and horizontally, each equipped with 12 antennas. The antennas transmit a waveform called FMCW \cite{stove1992linear} and sweep the frequencies from 5.4 to 7.2 GHz. Intuitively, the antenna arrays provide angular resolution and the FMCW provides depth resolution.

\label{sec:rf}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{rf-heatmap}
\caption{\footnotesize{RF heatmaps and an RGB image recorded at the same time.}}\label{fig:rf-heatmaps}
% \vspace{-5pt}
\vskip -5 pt
\end{figure}

Our input RF signal takes the form of two-dimensional heatmaps, one from the horizontal array and the other from the vertical array. As shown in Figure \ref{fig:rf-heatmaps}, the horizontal heatmap is similar to a depth heatmap projected on a plane parallel to the ground, and the vertical heatmap is similar to a depth heatmap projected on a plane perpendicular to the ground. Red parts in the figure correspond to large RF power, while blue parts correspond to small RF power.  The radio generates 30 pairs of heatmaps per second. 

RF signals are  different from vision data. They contain much less information than RGB images. This is because the wave-length of RF signals is few centimeters making it hard to capture objects' shape using RF signals; they may even totally miss small objects such as a pen or cellphone. However, the FMCW radio enables us to get a relatively high resolution on depth ($\sim$8cm), making it much easier to locate a person. We harness this property to better associate RF signals and floormaps in the same coordinate system.
